Almost anomalous dissipation in advection-diffusion of a divergence-free passive vector

We explore the advection-diffusion of a passive vector described by $\partial_t u + U \cdot \nabla u = - \nabla p + \nu \Delta u$, where both $U$ and $u$ are divergence-free velocity fields. We approach this equation from an input/output perspective, with $U$ as the input and $u$ as the output. This input/output viewpoint has been widely applied in recent studies on passive scalar equation, in the context of anomalous dissipation, mixing, optimal scalar transport, and nonuniqueness problems. What makes the passive vector equation considerably more challenging compared to the passive scalar equation is the lack of a Lagrangian perspective due to the presence of pressure. In this paper, rather than requiring $U$ and $u$ to be identical (as in the Navier-Stokes equation), we require $U$ and $u$ to be identical only in certain characteristics. We focus on the case where the characteristics in question are anomalous and enhanced dissipation. We study the advection-diffusion of a passive vector in a Couette flow configuration. The main result of this paper is a construction of the velocity field $U$ for which the energy dissipation scales as $(\log \nu^{-1})^{-2}$ such that the energy dissipation in velocity field $u$ scales at least as $(\log \nu^{-1})^{-2}$. This means that both $U$ and $u$ exhibit near-anomalous dissipation, where the rate of energy dissipation decreases more slowly than any power-law $\nu^{\alpha}$ for any $\alpha > 0$. The result in this paper is not just a mathematical construct; it closely resembles the behavior of turbulent flow in a channel. The $(\log \nu^{-1})^{-2}$ decrease of energy dissipation is predicted by phenomenological theories of wall-bounded turbulence, a prediction that has been extensively validated through experiments and numerical simulations.

==> introduction.tex <==
\section{Introduction}
\label{sec:Intro}
To do list:
\begin{enumerate}[label = (\roman*)]
\item the dimension needs to be $d$ everywhere in the text, we are using $n$ for the wavenumber. 
\end{enumerate}


Turbulence is ever-present: from flows in engineering, such as a wake behind a submarine, the boundary layer over an aircraft wing, and the swirl in an internal combustion engine, to flows in nature, such as convection in lakes, riffles on rivers, and currents over oceans. Turbulence can be found in flows at relatively small scales, such as blood flow in arteries and while mixing cream in a morning coffee, to flows at astrophysical scales, for instance, in accretion disks around stars or black holes. Because of their ubiquitous nature, progress in science and technology often hinges on progress in research on turbulent flows. 

\bigskip

Turbulent flows are characterized by a wide range of flow scales, intense mixing of scalar fields, high rates of momentum transport, and significant energy dissipation rates. A natural question to ask is how do turbulent flows achieve these 'extreme' properties? In particular, we want to identify what are the principal flow structures within a typical turbulent flow that are responsible for the characteristics mentioned above and how these structures interact and persist while adhering to known flow dynamics. The practical and scientific significance of these inquiries can hardly be overstated. For example, a thorough understanding of the principal components in a turbulent flow can facilitate the development of control strategies for drag reduction in flow past objects and can help us design more efficient heat exchangers. It can also enable us to identify the correct physical mechanisms driving efficient scalar transport in oceans or elucidate the enhanced angular transport required for star formation. 

\bigskip

While identifying the principal flow structures is crucial, merely conceptualizing how the flow should look like does not enable us to validate its accuracy. The primary reason is that the Navier-Stokes equations are nonlinear, making it exceedingly difficult to simply write down an analytical expression corresponding to a possible flow conceptualization and then verify if the expression satisfies the equation.
The goal of these notes is precisely to do the same \dots
%\citet{kumar2023nonuniqueness} and \citep{kumar2022three}
